NeAT: Learning Neural Implicit Surfaces with Arbitrary Topologies from Multi-view Images

Recent progress in neural implicit functions has set new state-of-the-art in reconstructing high-fidelity 3D shapes from a collection of images. However, these approaches are limited to closed surfaces as they require the surface to be represented by a signed distance field. In this paper, we propose NeAT, a new neural rendering framework that can learn implicit surfaces with arbitrary topologies from multi-view images. In particular, NeAT represents the 3D surface as a level set of a signed distance function (SDF) with a validity branch for estimating the surface existence probability at the query positions. We also develop a novel neural volume rendering method, which uses SDF and validity to calculate the volume opacity and avoids rendering points with low validity. NeAT supports easy field-to-mesh conversion using the classic Marching Cubes algorithm. Extensive experiments on DTU, MGN, and Deep Fashion 3D datasets indicate that our approach is able to faithfully reconstruct both watertight and non-watertight surfaces. In particular, NeAT significantly outperforms the state-of-the-art methods in the task of open surface reconstruction both quantitatively and qualitatively.

==> Figure/ablation_mask/ablation_mask.tex <==
\begin{figure}[htb]
    \begin{minipage}[t]{.2\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/placeholder.pdf}
        % \subcaption{Image 1.}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{.2\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/placeholder.pdf}
        % \subcaption{Image 2.}
    \end{minipage}  
    \label{fig:ablation_mask}
    \caption{Ablation study on mask regularization.}
\end{figure}

==> Figure/comparison_open_d3d/comparison_open_d3d.tex <==
\begin{figure*}[htb]
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/long_sleeve_upper/230/gt.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/long_sleeve_upper/230/ours.png}
    \end{minipage}  
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/long_sleeve_upper/230/neus.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/long_sleeve_upper/230/idr.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/long_sleeve_upper/252/gt.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/long_sleeve_upper/252/ours.png}
    \end{minipage}  
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/long_sleeve_upper/252/neus.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/long_sleeve_upper/252/idr.png}
    \end{minipage}
    \vspace{-0.5cm}
    \\
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/short_sleeve_upper/337/gt.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/short_sleeve_upper/337/ours.png}
    \end{minipage}  
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/short_sleeve_upper/337/neus.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/short_sleeve_upper/337/idr.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/short_sleeve_upper/40/gt.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/short_sleeve_upper/40/ours.png}
    \end{minipage}  
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/short_sleeve_upper/40/neus.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/short_sleeve_upper/40/idr.png}
    \end{minipage}
    \vspace{-0.0cm}
    \\
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=0.5\textwidth]{Figure/comparison_open_d3d/no_sleeve_upper/212/gt.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/no_sleeve_upper/212/ours.png}
    \end{minipage}  
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/no_sleeve_upper/212/neus.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/no_sleeve_upper/212/idr.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/no_sleeve_upper/323/gt.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/no_sleeve_upper/323/ours.png}
    \end{minipage}  
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/no_sleeve_upper/323/neus.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/no_sleeve_upper/323/idr.png}
    \end{minipage}
    \vspace{-0.0cm}
    \\
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/long_sleeve_dress/340/gt.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/long_sleeve_dress/340/ours.png}
    \end{minipage}  
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/long_sleeve_dress/340/neus.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/long_sleeve_dress/340/idr.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/long_sleeve_dress/222/gt.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/long_sleeve_dress/222/ours.png}
    \end{minipage}  
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/long_sleeve_dress/222/neus.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/long_sleeve_dress/222/idr.png}
    \end{minipage}
    \vspace{-0.0cm}
    \\
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/63/gt.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/63/ours.png}
    \end{minipage}  
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/63/neus.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/63/idr.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/314/gt.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/314/ours.png}
    \end{minipage}  
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/314/neus.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/314/idr.png}
    \end{minipage}
    \vspace{-0.0cm}
    \\
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/313/gt.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/313/ours.png}
    \end{minipage}  
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/313/neus.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/313/idr.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/320/gt.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/320/ours.png}
    \end{minipage}  
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/320/neus.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/320/idr.png}
    \end{minipage}
    \vspace{-0.0cm}
    \\
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/pants/315/gt.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/pants/315/ours.png}
    \end{minipage}  
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/pants/315/neus.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/pants/315/idr.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/pants/546/gt.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/pants/546/ours.png}
    \end{minipage}  
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/pants/546/neus.png}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/pants/546/idr.png}
    \end{minipage}
    \vspace{-0.0cm}
    \\
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \subfloat[GT]{\includegraphics[width=\textwidth]{Figure/comparison_open_d3d/skirts/164/gt.png}}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \subfloat[\modelName~ (Ours)]{\includegraphics[width=\textwidth]{Figure/comparison_open_d3d/skirts/164/ours.png}}
    \end{minipage}  
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \subfloat[NeuS]{\includegraphics[width=\textwidth]{Figure/comparison_open_d3d/skirts/164/neus.png}}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \subfloat[IDR]{\includegraphics[width=\textwidth]{Figure/comparison_open_d3d/skirts/164/idr.png}}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \subfloat[GT]{\includegraphics[width=\textwidth]{Figure/comparison_open_d3d/skirts/480/gt.png}}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \subfloat[\modelName~ (Ours)]{\includegraphics[width=\textwidth]{Figure/comparison_open_d3d/skirts/480/ours.png}}
    \end{minipage}  
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \subfloat[NeuS]{\includegraphics[width=\textwidth]{Figure/comparison_open_d3d/skirts/480/neus.png}}
    \end{minipage}
    \begin{minipage}[t]{.12\textwidth}
        \centering
        \subfloat[IDR]{\includegraphics[width=\textwidth]{Figure/comparison_open_d3d/skirts/480/idr.png}}
    \end{minipage}
\caption{Comparisons on open surface reconstruction. \modelName~is able to reconstruct high-fidelity open surfaces; while NeuS~\cite{wang2021neus} and IDR~\cite{yariv2020idr} reconstruct watertight surfaces.
% \weikai{(Update: I still think blue color is better -- pink looks a bit weird ...) We need a better rendering. Use more advanced renderer, i.e. blender, to render the double surfaces.}
}
\vspace{-2em}
\label{fig:comparison_open}
\end{figure*}

==> Figure/comparison_open_d3d/comparison_supp1.tex <==
\begin{figure*}[htb]
	\vspace{0.0mm}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/long_sleeve_upper/230/crop/gt_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/long_sleeve_upper/230/crop/gt.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/long_sleeve_upper/230/crop/ours_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/long_sleeve_upper/230/crop/ours.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/long_sleeve_upper/230/crop/neus_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/long_sleeve_upper/230/crop/neus.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/long_sleeve_upper/230/crop/idr_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/long_sleeve_upper/230/crop/idr.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/long_sleeve_upper/230/crop/HFS_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/long_sleeve_upper/230/crop/HFS.png}
	\end{minipage}
	\\
	\vspace{0.0mm}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/short_sleeve_upper/40/crop/gt_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/short_sleeve_upper/40/crop/gt.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/short_sleeve_upper/40/crop/ours_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/short_sleeve_upper/40/crop/ours.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/short_sleeve_upper/40/crop/neus_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/short_sleeve_upper/40/crop/neus.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/short_sleeve_upper/40/crop/idr_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/short_sleeve_upper/40/crop/idr.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/short_sleeve_upper/40/crop/HFS_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/short_sleeve_upper/40/crop/HFS.png}
	\end{minipage}
	\\
	\vspace{0.0mm}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/no_sleeve_upper/212/crop/gt_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/no_sleeve_upper/212/crop/gt.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/no_sleeve_upper/212/crop/ours_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/no_sleeve_upper/212/crop/ours.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/no_sleeve_upper/212/crop/neus_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/no_sleeve_upper/212/crop/neus.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/no_sleeve_upper/212/crop/idr_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/no_sleeve_upper/212/crop/idr.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/no_sleeve_upper/212/crop/HFS_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/no_sleeve_upper/212/crop/HFS.png}
	\end{minipage}
	\\
	\vspace{0.0mm}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/long_sleeve_dress/222/crop/gt_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/long_sleeve_dress/222/crop/gt.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/long_sleeve_dress/222/crop/ours_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/long_sleeve_dress/222/crop/ours.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/long_sleeve_dress/222/crop/neus_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/long_sleeve_dress/222/crop/neus.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/long_sleeve_dress/222/crop/idr_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/long_sleeve_dress/222/crop/idr.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/long_sleeve_dress/222/crop/HFS_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/long_sleeve_dress/222/crop/HFS.png}
	\end{minipage}
	\\
	\vspace{0.0mm}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/long_sleeve_dress/340/crop/gt_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/long_sleeve_dress/340/crop/gt.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/long_sleeve_dress/340/crop/ours_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/long_sleeve_dress/340/crop/ours.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/long_sleeve_dress/340/crop/neus_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/long_sleeve_dress/340/crop/neus.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/long_sleeve_dress/340/crop/idr_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/long_sleeve_dress/340/crop/idr.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/long_sleeve_dress/340/crop/HFS_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/long_sleeve_dress/340/crop/HFS.png}
	\end{minipage}
	\\
	\vspace{0.0mm}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/314/crop/gt_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/314/crop/gt.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/314/crop/ours_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/314/crop/ours.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/314/crop/neus_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/314/crop/neus.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/314/crop/idr_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/314/crop/idr.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/314/crop/HFS_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/314/crop/HFS.png}
	\end{minipage}
	\\
	\vspace{0.0mm}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/92/crop/gt_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/92/crop/gt.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/92/crop/ours_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/92/crop/ours.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/92/crop/neus_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/92/crop/neus.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/92/crop/idr_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/92/crop/idr.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/92/crop/HFS_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/92/crop/HFS.png}
	\end{minipage}
	\\
	\vspace{0.0mm}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/313/crop/gt_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/313/crop/gt.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/313/crop/ours_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/313/crop/ours.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/313/crop/neus_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/313/crop/neus.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/313/crop/idr_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/313/crop/idr.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/313/crop/HFS_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/313/crop/HFS.png}
	\end{minipage}
	\\
	\vspace{0.0mm}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/pants/546/crop/gt_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/pants/546/crop/gt.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/pants/546/crop/ours_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/pants/546/crop/ours.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/pants/546/crop/neus_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/pants/546/crop/neus.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/pants/546/crop/idr_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/pants/546/crop/idr.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/pants/546/crop/HFS_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/pants/546/crop/HFS.png}
	\end{minipage}
	\\
	\vspace{0.0mm}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\subfloat[GT]{\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/skirts/480/crop/gt_marked.png}}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/skirts/480/crop/gt.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\subfloat[Ours]{\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/skirts/480/crop/ours_marked.png}}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/skirts/480/crop/ours.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\subfloat[NeuS]{\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/skirts/480/crop/neus_marked.png}}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/skirts/480/crop/neus.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\subfloat[IDR]{\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/skirts/480/crop/idr_marked.png}}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/skirts/480/crop/idr.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\subfloat[HFS]{\includegraphics[width=0.9\textwidth]{Figure/comparison_open_d3d/skirts/480/crop/HFS_marked.png}}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_d3d/skirts/480/crop/HFS.png}
	\end{minipage}
\vspace{-1em}
\caption{Comparisons on open surface reconstruction of the \DFD~\cite{zhu2020deep}. NeAT is able to reconstruct high-fidelity open surfaces while NeuS~\cite{wang2021neus}, HF-NeuS~\cite{wang2022hfneus} and IDR~\cite{yariv2020idr} fail to recover the correct topologies.}
\vspace{-1em}
\label{fig:comparison_dfd_supp1}
\end{figure*}


==> Figure/comparison_open_d3d/comparison_supp2.tex <==
\begin{figure*}[htbp]
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/92/crop/gt_marked.png}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/92/crop/gt.png}
    \end{minipage}
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/92/crop/ours_marked.png}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/92/crop/ours.png}
    \end{minipage}
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/92/crop/neus_marked.png}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/92/crop/neus.png}
    \end{minipage}
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/92/crop/idr_marked.png}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/short_sleeve_dress/92/crop/idr.png}
    \end{minipage}
    \\
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/313/crop/gt_marked.png}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/313/crop/gt.png}
    \end{minipage}
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/313/crop/ours_marked.png}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/313/crop/ours.png}
    \end{minipage}
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/313/crop/neus_marked.png}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/313/crop/neus.png}
    \end{minipage}
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/313/crop/idr_marked.png}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/313/crop/idr.png}
    \end{minipage}
    \\
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/320/crop/gt_marked.png}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/320/crop/gt.png}
    \end{minipage}
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/320/crop/ours_marked.png}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/320/crop/ours.png}
    \end{minipage}
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/320/crop/neus_marked.png}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/320/crop/neus.png}
    \end{minipage}
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/320/crop/idr_marked.png}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/no_sleeve_dress/320/crop/idr.png}
    \end{minipage}
    \\
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{Figure/comparison_open_d3d/pants/546/crop/gt_marked.png}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        {\includegraphics[width=\textwidth]{Figure/comparison_open_d3d/pants/546/crop/gt.png}}
    \end{minipage}
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{Figure/comparison_open_d3d/pants/546/crop/ours_marked.png}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        {\includegraphics[width=\textwidth]{Figure/comparison_open_d3d/pants/546/crop/ours.png}}
    \end{minipage}
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{Figure/comparison_open_d3d/pants/546/crop/neus_marked.png}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        {\includegraphics[width=\textwidth]{Figure/comparison_open_d3d/pants/546/crop/neus.png}}
    \end{minipage}
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{Figure/comparison_open_d3d/pants/546/crop/idr_marked.png}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        {\includegraphics[width=\textwidth]{Figure/comparison_open_d3d/pants/546/crop/idr.png}}
    \end{minipage}
    \\
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{Figure/comparison_open_d3d/skirts/164/crop/gt_marked.png}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/skirts/164/crop/gt.png}
    \end{minipage}
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{Figure/comparison_open_d3d/skirts/164/crop/ours_marked.png}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/skirts/164/crop/ours.png}
    \end{minipage}
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{Figure/comparison_open_d3d/skirts/164/crop/neus_marked.png}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/skirts/164/crop/neus.png}
    \end{minipage}
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{Figure/comparison_open_d3d/skirts/164/crop/idr_marked.png}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/skirts/164/crop/idr.png}
    \end{minipage}
    \\
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \subfloat[GT]{\includegraphics[width=1.2\textwidth]{Figure/comparison_open_d3d/skirts/480/crop/gt_marked.png}}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/skirts/480/crop/gt.png}
    \end{minipage}
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \subfloat[Ours]{\includegraphics[width=1.2\textwidth]{Figure/comparison_open_d3d/skirts/480/crop/ours_marked.png}}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/skirts/480/crop/ours.png}
    \end{minipage}
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \subfloat[NeuS]{\includegraphics[width=1.2\textwidth]{Figure/comparison_open_d3d/skirts/480/crop/neus_marked.png}}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/skirts/480/crop/neus.png}
    \end{minipage}
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \subfloat[IDR]{\includegraphics[width=1.2\textwidth]{Figure/comparison_open_d3d/skirts/480/crop/idr_marked.png}}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        \includegraphics[width=\textwidth]{Figure/comparison_open_d3d/skirts/480/crop/idr.png}
    \end{minipage}
\caption{Comparisons on open surface reconstruction of the \DFD~\cite{zhu2020deep} (cont'd). \modelName~is able to reconstruct high-fidelity open surfaces while NeuS~\cite{wang2021neus} and IDR~\cite{yariv2020idr} fail to  recover the correct topologies.
% reconstruct watertight surfaces.
% \weikai{(Update: I still think blue color is better -- pink looks a bit weird ...) We need a better rendering. Use more advanced renderer, i.e. blender, to render the double surfaces.}
}
\vspace{-1.5em}
\label{fig:comparison_dfd_supp2}
\end{figure*}

==> Figure/comparison_open_mgn/comparison_supp1.tex <==
\begin{figure*}[htb]
	\vspace{0.0mm}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/TShirtNoCoat/125611500935128/crop/gt_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/TShirtNoCoat/125611500935128/crop/gt.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/TShirtNoCoat/125611500935128/crop/ours_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/TShirtNoCoat/125611500935128/crop/ours.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/TShirtNoCoat/125611500935128/crop/neus_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/TShirtNoCoat/125611500935128/crop/neus.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/TShirtNoCoat/125611500935128/crop/idr_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/TShirtNoCoat/125611500935128/crop/idr.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/TShirtNoCoat/125611500935128/crop/HFS_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/TShirtNoCoat/125611500935128/crop/HFS.png}
	\end{minipage}
	\\
	\vspace{0.0mm}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/TShirtNoCoat/125611504306885/crop/gt_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/TShirtNoCoat/125611504306885/crop/gt.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/TShirtNoCoat/125611504306885/crop/ours_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/TShirtNoCoat/125611504306885/crop/ours.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/TShirtNoCoat/125611504306885/crop/neus_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/TShirtNoCoat/125611504306885/crop/neus.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/TShirtNoCoat/125611504306885/crop/idr_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/TShirtNoCoat/125611504306885/crop/idr.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/TShirtNoCoat/125611504306885/crop/HFS_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/TShirtNoCoat/125611504306885/crop/HFS.png}
	\end{minipage}
	\\
	\vspace{0.0mm}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/ShirtNoCoat/125611517867589/crop/gt_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/ShirtNoCoat/125611517867589/crop/gt.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/ShirtNoCoat/125611517867589/crop/ours_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/ShirtNoCoat/125611517867589/crop/ours.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/ShirtNoCoat/125611517867589/crop/neus_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/ShirtNoCoat/125611517867589/crop/neus.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/ShirtNoCoat/125611517867589/crop/idr_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/ShirtNoCoat/125611517867589/crop/idr.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/ShirtNoCoat/125611517867589/crop/HFS_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/ShirtNoCoat/125611517867589/crop/HFS.png}
	\end{minipage}
	\\
	\vspace{0.0mm}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/ShirtNoCoat/125611502992247/crop/gt_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/ShirtNoCoat/125611502992247/crop/gt.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/ShirtNoCoat/125611502992247/crop/ours_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/ShirtNoCoat/125611502992247/crop/ours.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/ShirtNoCoat/125611502992247/crop/neus_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/ShirtNoCoat/125611502992247/crop/neus.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/ShirtNoCoat/125611502992247/crop/idr_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/ShirtNoCoat/125611502992247/crop/idr.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/ShirtNoCoat/125611502992247/crop/HFS_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/ShirtNoCoat/125611502992247/crop/HFS.png}
	\end{minipage}
	\\
	\vspace{0.0mm}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/LongCoat/125611504997669/crop/gt_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/LongCoat/125611504997669/crop/gt.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/LongCoat/125611504997669/crop/ours_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/LongCoat/125611504997669/crop/ours.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/LongCoat/125611504997669/crop/neus_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/LongCoat/125611504997669/crop/neus.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/LongCoat/125611504997669/crop/idr_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/LongCoat/125611504997669/crop/idr.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/LongCoat/125611504997669/crop/HFS_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/LongCoat/125611504997669/crop/HFS.png}
	\end{minipage}
	\\
	\vspace{0.0mm}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/LongCoat/125611520103063/crop/gt_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/LongCoat/125611520103063/crop/gt.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/LongCoat/125611520103063/crop/ours_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/LongCoat/125611520103063/crop/ours.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/LongCoat/125611520103063/crop/neus_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/LongCoat/125611520103063/crop/neus.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/LongCoat/125611520103063/crop/idr_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/LongCoat/125611520103063/crop/idr.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/LongCoat/125611520103063/crop/HFS_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/LongCoat/125611520103063/crop/HFS.png}
	\end{minipage}
	\\
	\vspace{0.0mm}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/Pants/125611487366942/crop/gt_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/Pants/125611487366942/crop/gt.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/Pants/125611487366942/crop/ours_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/Pants/125611487366942/crop/ours.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/Pants/125611487366942/crop/neus_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/Pants/125611487366942/crop/neus.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/Pants/125611487366942/crop/idr_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/Pants/125611487366942/crop/idr.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/Pants/125611487366942/crop/HFS_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/Pants/125611487366942/crop/HFS.png}
	\end{minipage}
	\\
	\vspace{0.0mm}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/Pants/125611522089953/crop/gt_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/Pants/125611522089953/crop/gt.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/Pants/125611522089953/crop/ours_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/Pants/125611522089953/crop/ours.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/Pants/125611522089953/crop/neus_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/Pants/125611522089953/crop/neus.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/Pants/125611522089953/crop/idr_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/Pants/125611522089953/crop/idr.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/Pants/125611522089953/crop/HFS_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/Pants/125611522089953/crop/HFS.png}
	\end{minipage}
	\\
	\vspace{0.0mm}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/ShortPants/125611504192867/crop/gt_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/ShortPants/125611504192867/crop/gt.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/ShortPants/125611504192867/crop/ours_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/ShortPants/125611504192867/crop/ours.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/ShortPants/125611504192867/crop/neus_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/ShortPants/125611504192867/crop/neus.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/ShortPants/125611504192867/crop/idr_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/ShortPants/125611504192867/crop/idr.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/ShortPants/125611504192867/crop/HFS_marked.png}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/ShortPants/125611504192867/crop/HFS.png}
	\end{minipage}
	\\
	\vspace{0.0mm}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\subfloat[GT]{\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/ShortPants/125611499279708/crop/gt_marked.png}}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/ShortPants/125611499279708/crop/gt.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\subfloat[Ours]{\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/ShortPants/125611499279708/crop/ours_marked.png}}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/ShortPants/125611499279708/crop/ours.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\subfloat[NeuS]{\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/ShortPants/125611499279708/crop/neus_marked.png}}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/ShortPants/125611499279708/crop/neus.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\subfloat[IDR]{\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/ShortPants/125611499279708/crop/idr_marked.png}}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/ShortPants/125611499279708/crop/idr.png}
	\end{minipage}
	\begin{minipage}[t]{0.13\textwidth}
		\centering
		\subfloat[HFS]{\includegraphics[width=0.9\textwidth]{Figure/comparison_open_mgn/ShortPants/125611499279708/crop/HFS_marked.png}}
	\end{minipage}
	\begin{minipage}[t]{0.06\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Figure/comparison_open_mgn/ShortPants/125611499279708/crop/HFS.png}
	\end{minipage}
\vspace{-1em}
\caption{Comparisons on open surface reconstruction of the \MGN~\cite{bhatnagar2019mgn}. NeAT is able to reconstruct high-fidelity open surfaces while NeuS~\cite{wang2021neus}, HF-NeuS~\cite{wang2022hfneus} and IDR~\cite{yariv2020idr} fail to recover the correct topologies.}
\vspace{-1em}
\label{fig:comparison_mgn_supp1}
\end{figure*}


==> Figure/comparison_open_mgn/comparison_supp2.tex <==
\begin{figure*}[htbp]
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{Figure/comparison_open_mgn/ShortPants/125611499279708/crop/gt_marked.png}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        \includegraphics[width=\textwidth]{Figure/comparison_open_mgn/ShortPants/125611499279708/crop/gt.png}
    \end{minipage}
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{Figure/comparison_open_mgn/ShortPants/125611499279708/crop/ours_marked.png}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        \includegraphics[width=\textwidth]{Figure/comparison_open_mgn/ShortPants/125611499279708/crop/ours.png}
    \end{minipage}
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{Figure/comparison_open_mgn/ShortPants/125611499279708/crop/neus_marked.png}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        \includegraphics[width=\textwidth]{Figure/comparison_open_mgn/ShortPants/125611499279708/crop/neus.png}
    \end{minipage}
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{Figure/comparison_open_mgn/ShortPants/125611499279708/crop/idr_marked.png}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        \includegraphics[width=\textwidth]{Figure/comparison_open_mgn/ShortPants/125611499279708/crop/idr.png}
    \end{minipage}
    \\
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{Figure/comparison_open_mgn/ShortPants/125611504192867/crop/gt_marked.png}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        \includegraphics[width=\textwidth]{Figure/comparison_open_mgn/ShortPants/125611504192867/crop/gt.png}
    \end{minipage}
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{Figure/comparison_open_mgn/ShortPants/125611504192867/crop/ours_marked.png}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        \includegraphics[width=\textwidth]{Figure/comparison_open_mgn/ShortPants/125611504192867/crop/ours.png}
    \end{minipage}
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{Figure/comparison_open_mgn/ShortPants/125611504192867/crop/neus_marked.png}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        \includegraphics[width=\textwidth]{Figure/comparison_open_mgn/ShortPants/125611504192867/crop/neus.png}
    \end{minipage}
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{Figure/comparison_open_mgn/ShortPants/125611504192867/crop/idr_marked.png}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        \includegraphics[width=\textwidth]{Figure/comparison_open_mgn/ShortPants/125611504192867/crop/idr.png}
    \end{minipage}
    \\
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{Figure/comparison_open_mgn/Pants/125611487366942/crop/gt_marked.png}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        \includegraphics[width=\textwidth]{Figure/comparison_open_mgn/Pants/125611487366942/crop/gt.png}
    \end{minipage}
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{Figure/comparison_open_mgn/Pants/125611487366942/crop/ours_marked.png}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        \includegraphics[width=\textwidth]{Figure/comparison_open_mgn/Pants/125611487366942/crop/ours.png}
    \end{minipage}
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{Figure/comparison_open_mgn/Pants/125611487366942/crop/neus_marked.png}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        \includegraphics[width=\textwidth]{Figure/comparison_open_mgn/Pants/125611487366942/crop/neus.png}
    \end{minipage}
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{Figure/comparison_open_mgn/Pants/125611487366942/crop/idr_marked.png}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        \includegraphics[width=\textwidth]{Figure/comparison_open_mgn/Pants/125611487366942/crop/idr.png}
    \end{minipage}
    \\
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \subfloat[GT]{\includegraphics[width=1.2\textwidth]{Figure/comparison_open_mgn/Pants/125611522089953/crop/gt_marked.png}}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        {\includegraphics[width=\textwidth]{Figure/comparison_open_mgn/Pants/125611522089953/crop/gt.png}}
    \end{minipage}
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \subfloat[Ours]{\includegraphics[width=1.2\textwidth]{Figure/comparison_open_mgn/Pants/125611522089953/crop/ours_marked.png}}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        {\includegraphics[width=\textwidth]{Figure/comparison_open_mgn/Pants/125611522089953/crop/ours.png}}
    \end{minipage}
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \subfloat[NeuS]{\includegraphics[width=1.2\textwidth]{Figure/comparison_open_mgn/Pants/125611522089953/crop/neus_marked.png}}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        {\includegraphics[width=\textwidth]{Figure/comparison_open_mgn/Pants/125611522089953/crop/neus.png}}
    \end{minipage}
    \begin{minipage}[t]{.16\textwidth}
        \centering
        \subfloat[IDR]{\includegraphics[width=1.2\textwidth]{Figure/comparison_open_mgn/Pants/125611522089953/crop/idr_marked.png}}
    \end{minipage}
    \begin{minipage}[t]{.08\textwidth}
        \vspace{-20mm}
        \hspace*{2mm}
        {\includegraphics[width=\textwidth]{Figure/comparison_open_mgn/Pants/125611522089953/crop/idr.png}}
    \end{minipage}
\caption{Comparisons on open surface reconstruction of the \MGN~\cite{bhatnagar2019mgn}. Row 1 -- 2 are evaluated on the \textit{ShortPants} category.  Row 3 - 4 are evaluated on the \textit{Pants} category. \modelName~is able to reconstruct high-fidelity open surfaces while NeuS~\cite{wang2021neus} and IDR~\cite{yariv2020idr} fail to  recover the correct topologies.
% reconstruct watertight surfaces.
% \weikai{(Update: I still think blue color is better -- pink looks a bit weird ...) We need a better rendering. Use more advanced renderer, i.e. blender, to render the double surfaces.}
}
\vspace{-1.5em}
\label{fig:comparison_mgn_supp2}
\end{figure*}

==> Figure/networks/rendering_network.tex <==
\begin{figure*}[t]
\centering
    \includegraphics[width=0.85\linewidth]{Figure/networks/image_rendering_network.pdf}
\caption{
The network structure of \textbf{Color-Net}. The units marked with solid lines are used in the multi- and single-view reconstruction experiment. The units marked with dotted lines are only used in the latter.
}
\vspace{-1em}
\label{fig:rendering_network}
\end{figure*}


==> Figure/networks/sdf_network.tex <==
\begin{figure*}[t]
\centering
    \includegraphics[width=0.85\linewidth]{Figure/networks/image_sdf_network.pdf}
\caption{
Left: the network structure of \textbf{SDF-Net}. Right: the network structure of \textbf{Validity-Net}. The units marked with solid lines are used in the multi- and single-view reconstruction experiment. The units marked with dotted lines are only used in the latter.
}
\vspace{-1em}
\label{fig:sdf_network}
\end{figure*}


==> Tables/comparison_open_mgn.tex <==
\begin{table}[htbp]
    \centering
    \begin{tabular}{|c|c|c|c|}
        \hline
        CD ($\times 10^{-3}$) & Ours & NeuS~\cite{wang2021neus} & IDR~\cite{yariv2020idr} \\
        \hline
        LongCoat & \textbf{5.561} & $7.361$ & $10.348$\\
        TShirtNoCoat & \textbf{TODO} & $TODO$ & $14.784$\\
        ShirtNoCoat & \textbf{4.843} & $6.135$ & $10.091$\\
        ShortPants & \textbf{TODO} & $TODO$ & $14.203$\\
        Pants & \textbf{TODO} & $TODO$ & $15.574$\\
        \hline
    \end{tabular}
    \caption{Quantitative evaluation on \MGN.}
    \label{table:comparison_open_mgn}
\end{table}
